Preventing Discriminatory Decision-making in Evolving Data Streams

Bias in machine learning has rightly received significant attention over the last decade. However, most fair machine learning (fair-ML) work to address bias in decision-making systems has focused solely on the offline setting. Despite the wide prevalence of online systems in the real world, work on identifying and correcting bias in the online setting is severely lacking. The unique challenges of the online environment make addressing bias more difficult than in the offline setting. First, Streaming Machine Learning (SML) algorithms must deal with the constantly evolving real-time data stream. Second, they need to adapt to changing data distributions (concept drift) to make accurate predictions on new incoming data. Adding fairness constraints to this already complicated task is not straightforward. In this work, we focus on the challenges of achieving fairness in biased data streams while accounting for the presence of concept drift, accessing one sample at a time. We present Fair Sampling over Stream ($FS^2$), a novel fair rebalancing approach capable of being integrated with SML classification algorithms. Furthermore, we devise the first unified performance-fairness metric, Fairness Bonded Utility (FBU), to evaluate and compare the trade-off between performance and fairness of different bias mitigation methods efficiently. FBU simplifies the comparison of fairness-performance trade-offs of multiple techniques through one unified and intuitive evaluation, allowing model designers to easily choose a technique. Overall, extensive evaluations show our measures surpass those of other fair online techniques previously reported in the literature.

==> sections/introduction.tex <==

\section{Introduction}
\label{sec:intro}

Machine learning (ML) systems, which benefits from the availability of large-scale datasets, 
have demonstrated great potential in tackling a wide range of critical tasks, e.g., human resource management~[xx], health cares~[xx], sentiment analysis~[xx], facial recognition~[xx], etc. 
For example, according to a report by Worldbank~[x], credit bureaus have been actively leveraging machine learning to conduct financial related activities, e.g., credit scoring, fraud detection, etc.
In addition, machine ML systems are also used in hiring like resume screening and candidate assessment. 
However, recent studies reveal the other side of the coin: \textit{ML systems can be biased}.
ML systems have been shown to be biased in various aspects, e.g., gender bias, race bias, etc.
An instance of gender bias in machine learning is that that state-of-the-art sentiment analysis tools tend to predict texts containing female names as negative~\cite{biasfinder}.
A deployed ML system for evaluating a defendant's risk of future crime was found to be biased against (i.e., producing high risk) black defendants~[x].

% So Fairness testing and bias mitigation are important. researchers have put a lot of effort.
% Introducing the state-of-the-art, and there disadvantage
The bias in ML systems can be harmful to the society, 
which has attracted attention from researchers in both software engineering and machine learning communities to uncover and mitigate the bias.




% We propose a novel method: xx. Explain our techincal design

% Evaluation Settings.

% Results

% Aspircational Contribution

% Structure of the paper

==> sections/rel_work.tex <==
\section{Related Work}
\label{sec:rel-work}
This section presents the two lines of works that are related to this study. 
ML systems are a subset of AI systems, so we first discuss the works related to AI testing.
Then, we discuss the works that are specific to testing and improving fairness in AI systems.

\subsection{AI Testing}

Although demonstrating the potential of tackling important tasks, AI systems still require sufficient amount of effort to ensure their quality from various aspects, including correctness, robustness, security, privacy, etc.

% Testing different systems (ASR, NLP, CV, RL, Code Models), different aspects (Correctness, robustness, security, performance, etc)
Researchers have built a wide range of tools to test various AI systems.
Motivated by the usage of code coverage metrics (e.g, line coverage, branch coverage, etc) in testing conventional software systems, 
Pei et al.~\cite{DeepXplore} propose DeepXplore, a tool that uses neuron coverage as a guidance to generate test cases for deep neural networks.
The following researchers extend this work by proposing structural neuron coverage metrics, e.g., neuron boundary coverage, etc. 
These metrics are the foundation for a series of AI testing tools, including DeepHunter~\cite{DeepHunter}, DeepGauge~\cite{DeepGauge}, DeepCT~\cite{DeepCT}, DeepTest~\cite{DeepTest}, etc.
However, recent studies~\cite{li2019structural,harel2020neuron,9376208,FSE_Yan,rl_coverage,9825775} also reveal that neuron coverage may not be effective enough to expose the vulnerabilities of AI systems.

% Different testing metrics. coverage driven, suprise adequacy, loss driven, etc.


\subsection{AI Fairness Testing and Improvement}

% Fairness testing.
